Spin-states in multiphoton pair production for circularly polarized light

Scalar and fermionic particle pair production in rotating electric fields is investigated in the nonperturbative multiphoton regime. Angular momentum distribution functions in above-threshold pair production processes are calculated numerically within quantum kinetic theory and discussed on the basis of a photon absorption model. The particle spectra can be understood if the spin states of the particle-antiparticle pair are taken into account.

==> TeX/Bibliography.tex <==

\bibliographystyle{unsrt}

\begin{thebibliography}{10}\setlength{\itemsep}{-0.5mm}

\bibitem{Reid} 
  K. L. Reid, 
  Annu. Rev. Phys. Chem. 2003. 54:397-424.
  %https://doi.org/10.1146/annurev.physchem.54.011002.103814
  
\bibitem{Brezin}
  E.~Brezin and C.~Itzykson,
  %``Pair production in vacuum by an alternating field,''
  Phys.\ Rev.\ D {\bf 2}, 1191 (1970);\\
  %%CITATION = PHRVA,D2,1191;%%
  %251 citations counted in INSPIRE as of 18 Oct 2013  
  V.~S.~Popov, Zh.\ Eksp.\ Teor.\ Fiz.\ {\bf 63}, 1586 (1972) [Sov.
  Phys. JETP 36, 840 (1973)]. 
  
\bibitem{Delone:1994}  
  N.~B.~Delone and V.~P.~Krainov, ``Multiphoton Processes in Atoms'', Springer 
  (Berlin) (1994);\\
  R.~Kopold, W.~Becker, M.~Kleber, G.~G.~Paulus,
  %``Channel-closing effects in high-order above-threshold ionizationand 
  %high-order harmonic generation,''
  J.\ Phys.\ B {\bf 35}, 217 (2002).
  %\cite{Brezin:1970xf}
  %\bibitem{Brezin:1970xf} 
  
%\cite{Kohlfurst:2013ura}
\bibitem{Kohlfurst:2013ura}
  C.~Kohlf\"urst, H.~Gies and R.~Alkofer,
  %``Effective mass signatures in multiphoton pair production,''
  Phys.\ Rev.\ Lett.\  {\bf 112} (2014) 050402
  [arXiv:1310.7836 [hep-ph]].
  %%CITATION = ARXIV:1310.7836;%%
  %19 citations counted in INSPIRE as of 11 Nov 2015    
   
%\cite{Lv:2018qxy}
\bibitem{Lv:2018qxy}
  Q.~Z.~Lv, S.~Dong, C.~Lisowski, R.~Pelphrey, Y.~T.~Li, Q.~Su and R.~Grobe,
  %``Quantum-mechanical approach to the laser-assisted vacuum decay,''
  Phys.\ Rev.\ A {\bf 97} (2018) no.5,  053416;\\
  %doi:10.1103/PhysRevA.97.053416
  %%CITATION = doi:10.1103/PhysRevA.97.053416;%%
  %1 citations counted in INSPIRE as of 30 Aug 2018  
 T.~W.~B. Kibble, A. Salam and J. A. Strathdee,
 Nucl. Phys. B 96, 255 (1975);\\
%\cite{Harvey:2012ie} 
  C.~Harvey, T.~Heinzl, A.~Ilderton and M.~Marklund,
  %``Intensity-Dependent Electron Mass Shift in a Laser Field: Existence, 
%Universality, and Detection,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 100402 (2012)
  [arXiv:1203.6077 [hep-ph]];\\
  %%CITATION = ARXIV:1203.6077;%%
  %8 citations counted in INSPIRE as of 30 Sep 2013    
  T.~W.~B.~Kibble,
  %``Mutual Refraction of Electrons and Photons,''
  Phys.\ Rev.\  {\bf 150}, 1060 (1966).
  %%CITATION = PHRVA,150,1060;%%
  %42 citations counted in INSPIRE as of 14 Oct 2013  
  
%\cite{Otto:2014ssa}
\bibitem{Otto:2014ssa}
  A.~Otto, D.~Seipt, D.~Blaschke, B.~K\"ampfer and S.~A.~Smolyansky,
  %``Lifting shell structures in the dynamically assisted Schwinger effect in periodic fields,''
  Phys.\ Lett.\ B {\bf 740} (2015) 335
  %doi:10.1016/j.physletb.2014.12.010
  [arXiv:1412.0890 [hep-ph]];\\
  %%CITATION = doi:10.1016/j.physletb.2014.12.010;%%
  %27 citations counted in INSPIRE as of 31 Jan 2018      
%\cite{Otto:2015gla}
%\bibitem{Otto:2015gla}
  A.~Otto, D.~Seipt, D.~Blaschke, S.~A.~Smolyansky and B.~K\"ampfer,
  %``Dynamical Schwinger process in a bifrequent electric field of finite duration: survey on amplification,''
  Phys.\ Rev.\ D {\bf 91} (2015) no.10,  105018
  %doi:10.1103/PhysRevD.91.105018
  [arXiv:1503.08675 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.91.105018;%%
  %32 citations counted in INSPIRE as of 12 Oct 2018
  
%\cite{Akal:2014eua}
\bibitem{Akal:2014eua}
  I.~Akal, S.~Villalba-Ch\'{a}vez and C.~M\"uller,
  %``Electron-positron pair production in a bifrequent oscillating electric field,''
  Phys.\ Rev.\ D {\bf 90} (2014) no.11,  113004
  %doi:10.1103/PhysRevD.90.113004
  [arXiv:1409.1806 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.113004;%%
  %44 citations counted in INSPIRE as of 04 Dec 2018  
  
\bibitem{IonizeH}
  Y. Gontier and M. Trahin, 
  %Multiphoton Ionization of Atomic Hydrogen in the Ground State
  Phys. Rev. {\bf 172} 83-87 (1968);\\
  Y. Gontier and N. K. Rahman and M. Trahin,
  %Angular Distribution of above-Threshold Ionization of Atomic Hydrogen
  Europhysics Letters {\bf 5} (7), 595, (1988);\\
  S. Dionissopoulou, Th. Mercouris, A. Lyras and  C. A. Nicolaides,
  %Strong laser-field effects in hydrogen:mHigh-order above-threshold ionization and photoelectron angular distributions
  Phys.\ Rev.\ A {\bf 55} (1997) 6,  4397.
  %10.1103/PhysRevA.55.4397  

\bibitem{PhysRevA.87.033413}
  Y. Huismans, A. Rouz\'ee, A. Gijsbertsen, P. S. W. M. Logman, F. L\'epine, C. Cauchy, S. Zamith, A. S. Stodolna, J. H. Jungmann, J. M. Bakker, G. Berden,
  B. Redlich, A. F. G. van der Meer, K. J. Schafer and M. J. J. Vrakking,
  Phys.\ Rev.\ A {\bf 87} (2013) 10, 033413.
  %10.1103/PhysRevA.87.033413  
 
\bibitem{Sauter:1931zz} 
  F.~Sauter,
  %``Uber das Verhalten eines Elektrons im homogenen elektrischen Feld nach der
%relativistischen Theorie Diracs,''
  Z.\ Phys.\  {\bf 69}, 742 (1931);\\
  %%CITATION = ZEPYA,69,742;%%
  %243 citations counted in INSPIRE as of 30 Sep 2013
  W.~Heisenberg and H.~Euler,
  %``Consequences of Dirac's theory of positrons,''
  Z.\ Phys.\  {\bf 98}, 714 (1936);\\
  %[physics/0605038].
  %%CITATION = PHYSICS/0605038;%%
  %901 citations counted in INSPIRE as of 30 Sep 2013  
  J.~S.~Schwinger,
  %``On gauge invariance and vacuum polarization,''
  Phys.\ Rev.\  {\bf 82}, 664 (1951). 
  %%CITATION = PHRVA,82,664;%%
  %3320 citations counted in INSPIRE as of 30 Sep 2013 
  
%\cite{Breit:1934zz}
\bibitem{Breit:1934zz}
  G.~Breit and J.~A.~Wheeler,
  %``Collision of Two Light Quanta,''
  Phys.\ Rev.\  {\bf 46} (1934) 1087.
  %doi:10.1103/PhysRev.46.1087
  %%CITATION = doi:10.1103/PhysRev.46.1087;%%
  %169 citations counted in INSPIRE as of 10 Oct 2018  

%\cite{Dinu:2017uoj}
\bibitem{Dinu:2017uoj}
  V.~Dinu and G.~Torgrimsson,
  %``Trident pair production in plane waves: Coherence, exchange, and spacetime inhomogeneity,''
  Phys.\ Rev.\ D {\bf 97} (2018) no.3,  036021
  %doi:10.1103/PhysRevD.97.036021
  [arXiv:1711.04344 [hep-ph]];\\
  %%CITATION = doi:10.1103/PhysRevD.97.036021;%%
  %7 citations counted in INSPIRE as of 10 Oct 2018  
%\cite{Mackenroth:2018smh}
%\bibitem{Mackenroth:2018smh}
  F.~Mackenroth and A.~Di Piazza,
  %``Nonlinear trident pair production in an arbitrary plane wave: a focus on the properties of the transition amplitude,''
  arXiv:1805.01731 [hep-ph].
  %%CITATION = ARXIV:1805.01731;%%
  %1 citations counted in INSPIRE as of 04 Dec 2018  
  
%\cite{Schutzhold:2008pz}
\bibitem{Schutzhold:2008pz}
  R.~Schutzhold, H.~Gies and G.~Dunne,
  %``Dynamically assisted Schwinger mechanism,''
  Phys.\ Rev.\ Lett.\  {\bf 101} (2008) 130404
  %doi:10.1103/PhysRevLett.101.130404
  [arXiv:0807.0754 [hep-th]].
  %%CITATION = doi:10.1103/PhysRevLett.101.130404;%%
  %173 citations counted in INSPIRE as of 10 Oct 2018  
%\cite{Torgrimsson:2017pzs}
%\bibitem{Torgrimsson:2017pzs}
  G.~Torgrimsson, C.~Schneider, J.~Oertel and R.~Sch\"utzhold,
  %``Dynamically assisted Sauter-Schwinger effect — non-perturbative versus perturbative aspects,''
  JHEP {\bf 1706} (2017) 043
  %doi:10.1007/JHEP06(2017)043
  [arXiv:1703.09203 [hep-th]].
  %%CITATION = doi:10.1007/JHEP06(2017)043;%%
  %12 citations counted in INSPIRE as of 10 Oct 2018  
%\cite{Kohlfurst:2012rb}
%\bibitem{Kohlfurst:2012rb}
  C.~Kohlfurst, M.~Mitter, G.~von Winckel, F.~Hebenstreit and R.~Alkofer,
  %``Optimizing the pulse shape for Schwinger pair production,''
  Phys.\ Rev.\ D {\bf 88} (2013) 045028
  %doi:10.1103/PhysRevD.88.045028
  [arXiv:1212.1385 [hep-ph]];\\
  %%CITATION = doi:10.1103/PhysRevD.88.045028;%%
  %38 citations counted in INSPIRE as of 10 Oct 2018  
%\cite{Aleksandrov:2017owa}
%\bibitem{Aleksandrov:2017owa}
  I.~A.~Aleksandrov, G.~Plunien and V.~M.~Shabaev,
  %``Pulse shape effects on the electron-positron pair production in strong laser fields,''
  Phys.\ Rev.\ D {\bf 95} (2017) no.5,  056013
  %doi:10.1103/PhysRevD.95.056013
  [arXiv:1701.01058 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.95.056013;%%
  %7 citations counted in INSPIRE as of 12 Oct 2018
  
%\cite{Burke:1997ew}
\bibitem{Burke:1997ew}
  D.~L.~Burke (SLAC)  {\it et al.},
%, R.~C.~Field, G.~Horton-Smith, T.~Kotseroglou, J.~E.~Spencer,
%D.~Walz, S.~C.~Berridge and W.~M.~Bugg {\it et al.},
  %``Positron production in multi - photon light by light scattering,''
  Phys.\ Rev.\ Lett.\  {\bf 79}, 1626 (1997);\\
  %%CITATION = PRLTA,79,1626;%%
  %194 citations counted in INSPIRE as of 26 Nov 2014
  C. Bamber {\it et al.}, 
%S. J. Boege, T. Koffas, T. Kotseroglou, A. C. Melissinos, D. D. 
%Meyerhofer {\it et al.},
  %Studies of nonlinear QED in collisions of 46.6 GeV electrons with intense
%laser pulses
  Phys. Rev. D {\bf 60}, 092004 (1999).    
  
\bibitem{Experiments}
  X.-L.~Zhu, T.-P. Yu, Z.-M. Sheng, Y. Yin, I. C. E. Turcu and A. Pukhov,
  Nat Commun. 2016; 7: 13686.   
  
%\cite{Ribeyre:2015fta}
\bibitem{Ribeyre:2015fta}
  X.~Ribeyre, M.~Lobet, E.~D'Humi\`{e}res, S.~Jequier, V.~T.~Tikhonchuk and O.~Jansen,
  %``Pair creation in collision of γ-ray beams produced with high-intensity lasers,''
  Phys.\ Rev.\ E {\bf 93} (2016) no.1,  013201
  %doi:10.1103/PhysRevE.93.013201
  [arXiv:1504.07868 [physics.ins-det]];\\
  %%CITATION = doi:10.1103/PhysRevE.93.013201;%%
  %13 citations counted in INSPIRE as of 14 Aug 2018
%\cite{Ringwald:2001ib}
%\bibitem{Ringwald:2001ib}
  A.~Ringwald,
  %``Pair production from vacuum at the focus of an X-ray free electron laser,''
  Phys.\ Lett.\ B {\bf 510} (2001) 107
  [hep-ph/0103185]; \\
  %%CITATION = HEP-PH/0103185;%%
  %135 citations counted in INSPIRE as of 26 Nov 2014     
  %O.~J.~Pike, F.~Mackenroth, E.~G.~Hill and S.~J.~Rose,
  %``A photon–photon collider in a vacuum hohlraum,''
  O.~J.~Pike, F.~Mackenroth, E.~G.~Hill and S.~J.~Rose, 
  Nature Photon. 8, 434-436 (2014); \\
  %1 citations counted in INSPIRE as of 26 Nov 2014    
%\bibitem{Sokolov:2010am}
  I.~V.~Sokolov, N.~M.~Naumova, J.~A.~Nees and G.~A.~Mourou,
  %``Pair Creation in QED-Strong Pulsed Laser Fields Interacting with Electron Beams,''
  Phys.\ Rev.\ Lett.\  {\bf 105} (2010) 195005
  %doi:10.1103/PhysRevLett.105.195005
  [arXiv:1009.0703 [physics.plasm-ph]];\\
  %%CITATION = doi:10.1103/PhysRevLett.105.195005;%%
  %53 citations counted in INSPIRE as of 14 Aug 2018  
%\cite{Hu:2010ye}
%\bibitem{Hu:2010ye}
  H.~Hu, C.~Muller and C.~H.~Keitel,
  %``Complete QED theory of multiphoton trident pair production in strong laser fields,''
  Phys.\ Rev.\ Lett.\  {\bf 105} (2010) 080401
  %doi:10.1103/PhysRevLett.105.080401
  [arXiv:1002.2596 [physics.atom-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.105.080401;%%
  %64 citations counted in INSPIRE as of 30 Aug 2018  
 
 %\cite{Vasak:1987um}
\bibitem{Vasak:1987umA}
  D.~Vasak, M.~Gyulassy and H.~T.~Elze,
  %``Quantum Transport Theory for Abelian Plasmas,''
  Annals Phys.\  {\bf 173} (1987) 462;\\
%\bibitem{Vasak:1987umB}  
  %%CITATION = APNYA,173,462;%%
  %55 citations counted in INSPIRE as of 19 Nov 2014   
%\bibitem{BB}
  I. Bialynicki-Birula, P. G\'ornicki and J. Rafelski, 
  Phys. Rev. D 44 (1991).    
  
\bibitem{Heinz}
%\bibitem{Zhuang:1998bqx}
  P.~f.~Zhuang and U.~W.~Heinz,
  %``Equal-Time Hierarchies in Quantum Transport Theory,''
  Phys.\ Rev.\ D {\bf 57} (1998) 6525
  %doi:10.1103/PhysRevD.57.6525
  [hep-ph/9610438, hep-ph/9801221];\\
  %%CITATION = doi:10.1103/PhysRevD.57.6525;%%
  %22 citations counted in INSPIRE as of 30 Aug 2018  
%\cite{Zhuang:1995pd}
%\bibitem{Zhuang:1995pd}
  P.~Zhuang and U.~W.~Heinz,
  %``Relativistic quantum transport theory for electrodynamics,''
  Annals Phys.\  {\bf 245} (1996) 311
  %doi:10.1006/aphy.1996.0011
  [nucl-th/9502034]; \\
  %%CITATION = doi:10.1006/aphy.1996.0011;%%
  %36 citations counted in INSPIRE as of 30 Aug 2018
%\cite{Ochs:1998qj}
%\bibitem{Ochs:1998qj}
  S.~Ochs and U.~W.~Heinz,
  %``Wigner functions in covariant and single time formulations,''
  Annals Phys.\  {\bf 266} (1998) 351
  %doi:10.1006/aphy.1998.5796
  [hep-th/9806118].
  %%CITATION = doi:10.1006/aphy.1998.5796;%%
  %30 citations counted in INSPIRE as of 30 Aug 2018
  
 %\cite{Smolyansky:1997fc}
\bibitem{Smolyansky:1997fc} 
  S.~A.~Smolyansky, G.~Ropke, S.~M.~Schmidt, D.~Blaschke, V.~D.~Toneev and
A.~V.~Prozorkevich,
  %``Dynamical derivation of a quantum kinetic equation for particle production
%in the Schwinger mechanism,''
  hep-ph/9712377;\\
  %%CITATION = HEP-PH/9712377;%%
  %30 citations counted in INSPIRE as of 16 Oct 2013
  Y.~Kluger, E.~Mottola and J.~M.~Eisenberg,
  %``The Quantum Vlasov equation and its Markov limit,''
  Phys.\ Rev.\ D {\bf 58}, 125015 (1998)
  [hep-ph/9803372];\\
  %%CITATION = HEP-PH/9803372;%%
  %87 citations counted in INSPIRE as of 16 Oct 2013  
  S.~M.~Schmidt, D.~Blaschke, G.~Ropke, S.~A.~Smolyansky, A.~V.~Prozorkevich and
V.~D.~Toneev,
  %``A Quantum kinetic equation for particle production in the Schwinger
%mechanism,''
  Int.\ J.\ Mod.\ Phys.\ E {\bf 7}, 709 (1998);
  [hep-ph/9809227];\\
  %%CITATION = HEP-PH/9809227;%%
  %72 citations counted in INSPIRE as of 30 Sep 2013   
  J.~C.~R.~Bloch, V.~A.~Mizerny, A.~V.~Prozorkevich, C.~D.~Roberts,
S.~M.~Schmidt, S.~A.~Smolyansky and D.~V.~Vinnik,
  %``Pair creation: Back reactions and damping,''
  Phys.\ Rev.\ D {\bf 60} (1999) 116011
  [nucl-th/9907027].
  %%CITATION = NUCL-TH/9907027;%%
  %57 citations counted in INSPIRE as of 26 Nov 2014     
  
%\cite{Li:2015cea}
\bibitem{Li:2015cea}
  Z.~L.~Li, D.~Lu and B.~S.~Xie,
  %``Effects of electric field polarizations on pair production,''
  Phys.\ Rev.\ D {\bf 92} (2015) no.8,  085001
  %doi:10.1103/PhysRevD.92.085001
  [arXiv:1508.03440 [quant-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.085001;%%
  %6 citations counted in INSPIRE as of 30 Aug 2018    
  
\bibitem{Rotating}
 A.~Blinne and H.~Gies,
  %``Pair Production in Rotating Electric Fields,''
  Phys.\ Rev.\ D {\bf 89} (2014), 085001
  [arXiv:1311.1678 [hep-ph]];\\
  %%CITATION = ARXIV:1311.1678;%%
  %4 citations counted in INSPIRE as of 26 Nov 2014  
  %\cite{Blinne:2016yzv}
%\bibitem{Blinne:2016yzv}
  A.~Blinne,
  %``Electron Positron Pair Production in Strong Electric Fields,''
  arXiv:1701.00743 [physics.plasm-ph].
  %%CITATION = ARXIV:1701.00743;%%
  %1 citations counted in INSPIRE as of 31 Aug 2018

%\cite{Blinne:2015zpa}
\bibitem{Blinne:2015zpa}
  A.~Blinne and E.~Strobel,
  %``Comparison of semiclassical and Wigner function methods in pair production in rotating fields,''
  Phys.\ Rev.\ D {\bf 93} (2016) no.2,  025014
  %doi:10.1103/PhysRevD.93.025014
  [arXiv:1510.02712 [hep-th]];\\
  %%CITATION = doi:10.1103/PhysRevD.93.025014;%%
  %11 citations counted in INSPIRE as of 28 Sep 2018  
%\cite{Li:2017qwd}
%\bibitem{Li:2017qwd}
  Z.~L.~Li, Y.~J.~Li and B.~S.~Xie,
  %``Momentum Vortices on Pairs Production by Two Counter-Rotating Fields,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.7,  076010
  %doi:10.1103/PhysRevD.96.076010
  [arXiv:1707.01353 [quant-ph]];\\
  %%CITATION = doi:10.1103/PhysRevD.96.076010;%%
  %1 citations counted in INSPIRE as of 30 Aug 2018
%\cite{Fillion-Gourdeau:2017uss}
%\bibitem{Fillion-Gourdeau:2017uss}
  F.~Fillion-Gourdeau, F.~Hebenstreit, D.~Gagnon and S.~MacLean,
  %``Pulse shape optimization for electron-positron production in rotating fields,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.1,  016012
  %doi:10.1103/PhysRevD.96.016012
  [arXiv:1704.08919 [hep-ph]];\\
  %%CITATION = doi:10.1103/PhysRevD.96.016012;%%
  %4 citations counted in INSPIRE as of 30 Aug 2018  
%\cite{Bulanov:2003aj}
%\bibitem{Bulanov:2003aj}
  S.~S.~Bulanov,
  %``The Pair production by circularly polarized electromagnetic wave in plasma,''
  Phys.\ Rev.\ E {\bf 69} (2004) 036408
  %doi:10.1103/PhysRevE.69.036408
  [hep-ph/0307296].
  %%CITATION = doi:10.1103/PhysRevE.69.036408;%%
  %22 citations counted in INSPIRE as of 04 Oct 2018     
  
\bibitem{NR}
  W. H. Press, S. A. Teukolsky, W. T. Vetterling and B. P. Flannery,
  Cambridge University Press,
  ISBN-13: 978-0521880688.     
  
%\cite{Yang:1948nq}
\bibitem{Yang:1948nq}
  C.~N.~Yang,
  %``On the Angular Distribution in Nuclear Reactions and Coincidence Measurements,''
  Phys.\ Rev.\  {\bf 74} (1948) 764.
  %doi:10.1103/PhysRev.74.764
  %%CITATION = doi:10.1103/PhysRev.74.764;%%
  %18 citations counted in INSPIRE as of 28 Sep 2018
  
%\cite{Marinov:1977gq}
\bibitem{Marinov:1977gq}
  M.~S.~Marinov and V.~S.~Popov,
  %``Electron-Positron Pair Creation from Vacuum Induced by Variable Electric Field,''
  Fortsch.\ Phys.\  {\bf 25} (1977) 373.
  %doi:10.1002/prop.19770250111
  %%CITATION = doi:10.1002/prop.19770250111;%%
  %88 citations counted in INSPIRE as of 28 Sep 2018  

\end{thebibliography}


==> TeX/Conclusion.tex <==
\paragraph{Discussion.--}

Particle pair production is a complex process and observables are very sensitive to changes in the background fields.
Nevertheless, it seems as if we have found a way to understand certain features of multiphoton pair production intuitively.

The specific procedure in which we obtained the particle creation rates $M_i$ is, in its current form, only applicable to purely circularly polarized fields.
Although the generic model \eqref{equ:I} can be applied for arbitrary field configurations, the composition of the particle spectra in terms
of angular momentum contributions takes on the particularly simple form \eqref{I_c} only in case of rotating fields.
For linearly polarized light, for example, the particles final angular momentum becomes a sum over many terms, because the
initial photons could have been left- or right-handed.

Our model is also limited to the nonperturbative multiphoton regime in pair production for Keldysh parameter $\gamma_\omega = \omega / \left(m \varepsilon \right) > 1$.
Moreover, the studied momentum signatures only emerge for multi-cycle pulses $\omega \tau \gg 1$. In a few-cycle pulse, the individual photon energies 
are varying too much, thus the clear characteristic peaks cannot form in the final particle spectrum. 

Another issue arises in experimental studies of pair production, e.g., the collision of two laser pulses at an arbitrary angle.
In such a case the photons carry momentum, thus linear momentum conservation has to be taken into account effectively excluding
some processes. Nevertheless, the way to interpret the momentum shells does not change.

Finally, charge-conjugation and parity invariance pose additional constraints on multiphoton pair production. 
For an even (odd) number of photons $n$, the (scalar) momentum distribution has to vanish for vanishing momentum $\mathbf{p}$ independent of the polarization of the incoming beams.
These constraints become especially important for linearly polarized fields, where, in principle, the angular momentum transfer-picture allows for
pair production at $\mathbf{p}=0$ for higher photon numbers. Within the context of this work, the model coincides with all selection rules.

\paragraph{Summary.--}

We have demonstrated that, in multiphoton pair production, the distribution functions for scalar and spin one-half particles in rotating electric fields
follow a specific, intuitive pattern. On the basis of accurate numerical solutions of quantum kinetic theory it is straightforward to obtain the spin-dependent particle
creation amplitudes. Although the procedure presented in this article is based on circularly polarized waves, the underlaying model 
can be readily extended to arbitrary field configurations.

\paragraph{Acknowledgments.--}

We thank Andr\'e Sternbeck, Holger Gies, Alexander Blinne and Greger Torgrimsson for interesting discussions.
We thank Holger Gies and Se\'{a}n Gray for a critical reading of the manuscript.
The work of C.K.~is funded by the Helmholtz Association through the
Helmholtz Postdoc Programme (PD-316). We acknowledge support by the
BMBF under grant No. 05P15SJFAA (FAIR-APPA-SPARC).

%Computations were performed on the ``Supermicro Server 1028TR-TF'' in Jena, which
%was funded by the Helmholtz Postdoc Programme (PD-316).




==> TeX/Foundations.tex <==
%\section{Theoretical Foundations}
\paragraph{Electric field pulse.--}

In order to study pair production for circularly polarized light, we have chosen the following model for the vector potential
\begin{equation}
 \mathbf{A} \left( t \right) =  -\frac{\varepsilon E_{cr}}{2\omega} \exp{ \left(-\frac{t^2}{\tau^2} \right) } 
 \begin{pmatrix}
  \sin \left( \omega t \right) \\
  \cos \left( \omega t \right) \\
  0
 \end{pmatrix}         ,
 \label{eq:A}
\end{equation}
with the critical field strength $E_{cr}=m^2/e$, the peak field strength $\varepsilon$, the pulse length $\tau$ and the photon energy $\omega$. 
The electric field is derived from this expression.

We have chosen the model \eqref{eq:A} to mimic a standing wave formed by two counter-propagating laser beams with propagation
direction $\pm \mathbf{\hat z}$. To form a standing wave pattern as given by eq. \eqref{eq:A} one beam has
to be left-handed and the other must be right-handed. As photons are spin-1 bosons we assume without loss of generality the
helicity to be quantum. Hence, every photon not only transfers an energy quant of $\omega$ to the particle-antiparticle pair, but also
increases its total angular momentum by one. 
%\footnote{All arguments still hold when the propagation directions of the fields are swapped with each other as
%only the (angular) momentum vector switches sign.} 

\paragraph{Quantum Kinetic Theory.--}

All numerical results are based upon a phase-space approach belonging to a particular class
of quantum kinetic theories. As we perform calculations for spatially homogeneous fields the governing equations of motion
take on a numerically favorable form. As a result, we are able to obtain very accurate numerical solutions allowing us to compare
the computed data with predictions from the model.

In the Weyl gauge, the quantum kinetic equations for spin-$1/2$ particles can be written as \cite{Rotating}
\begin{alignat}{5}
    & \partial_{t} \mathbbm{s}^v    && && -2 \mathbf{p} \br{t} \cdot \mathbbm{t_1}^v && &&= 
      - 2 \frac{ \ Q \br{t} }{ \omega \br{t}}, \\    
    & \partial_{t} \boldsymbol{\mathbbm{v}}^v && && +2\mathbf{p} \br{t} \times \boldsymbol{\mathbbm{a}}^v && +2\mathbbm{t_1}^v &&= 
       2 \frac{ e \mathbf{E} \br{t} - Q \br{t} \mathbf{p} \br{t} }{\omega \br{t}}, \\    
    & \partial_{t} \boldsymbol{\mathbbm{a}}^v && && +2 \mathbf{p} \br{t} \times \boldsymbol{\mathbbm{v}}^v && &&= \mathbf{0},  \\
    & \partial_{t} \boldsymbol{\mathbbm{t_1}}^v && && +2 \mathbf{p} \br{t} \ \mathbbm{s}^v && -2 \boldsymbol{\mathbbm{v}}^v &&= \mathbf{0}  
\end{alignat}
%introduced initial conditions as -1 p/w
with initial conditions
\begin{align}
  \mathbbm{s}_i^v = 0,\quad \boldsymbol{\mathbbm{v}}^v_{i} = \boldsymbol{\mathbbm{a}}^v_{i} = \boldsymbol{\mathbbm{t_1}}^v_{i} = \mathbf{0}.
\end{align}  
Following Refs. \cite{Vasak:1987umA, Heinz} we can associate the individual terms in the differential equation as mass density $\mathbbm{s}^v$, 
current density $\boldsymbol{\mathbbm{v}}^v$, spin density $\boldsymbol{\mathbbm{a}}^v$ and magnetic moment density $\boldsymbol{\mathbbm{t_1}}^v$.
We have used abbreviations for the one-particle energy $\omega \br{t} = \sqrt{1+ \mathbf{p} \br{t}^2}$, 
the kinetic momentum $\mathbf{p} \br{t} = \mathbf{q} -e \mathbf{A} \br{t} $ and the auxiliary variable 
$Q \br{t} = \dfrac{ e \mathbf{E} \br{t} \cdot \mathbf{p} \br{t} }{ \omega \br{t}^2}$. 

The equations of motion for scalar particles, on the other hand, are given by \cite{Heinz}
\begin{alignat}{5}
    & \partial_{t} \mathbbm{f}^v    && &&  -\mathbf{p} \br{t}^2 \left( \mathbbm{g}^v + \mathbbm{h}^v \right) && -2 \mathbbm{g}^v &&= 
      2 \frac{\mathbf{p} \br{t}^2}{\omega \br{t}}, \label{eq:sQED1} \\   
    & \partial_{t} \mathbbm{g}^v    && &&  +\mathbf{p} \br{t}^2 \mathbbm{f}^v && +2 \mathbbm{f}^v &&= 
      -\frac{1}{2} \frac{\left(1+ \omega \br{t}^2 \right) Q \br{t} }{\omega \br{t}}, \\   
    & \partial_{t} \mathbbm{h}^v    && &&  -\mathbf{p} \br{t}^2 \mathbbm{f}^v && &&= 
      -\frac{1}{2} \frac{\mathbf{p} \br{t}^2 Q \br{t} }{\omega \br{t}}.  \label{eq:sQED3}       
\end{alignat}
Again, the initial conditions have been incorporated into the equations of motion, thus
\begin{align}
  \mathbbm{f}_i^v = \mathbbm{g}_i^v = \mathbbm{h}_i^v = 0.
\end{align}  
From Refs. \cite{Heinz} we know to identify $\boldsymbol{\mathbbm{j}}^v = \mathbf{p} \br{t} \left( \mathbbm{g}^v + \mathbbm{h}^v \right)$ as current density and 
$\mathbbm{h}^v$ as mass density. The term $\mathbbm{f}^v$ does not seem to have a direct physical interpretation.

The time integration was performed using a Dormand-Prince Runge-Kutta integrator of order 8(5,3) \cite{NR}.
% Equations for sQED
% \begin{alignat}{5}
%     & \partial_{t} \mathbbm{f}    && && -Q \br{t} \mathbbm{g} && &&= 0, \\    
%     & \partial_{t} \mathbbm{g} && && -Q \br{t} \mathbbm{f} && +2 \omega \br{t} \mathbbm{h} &&= Q \br{t},\\    
%     & \partial_{t} \mathbbm{h} && && && -2 \omega \br{t} \mathbbm{g} &&= 0,
% \end{alignat}

Throughout this article we will discuss the results on the basis of the spin-dependent particle number density $f_s$, which is evaluated at asymptotic times. 
Hereby, the electron-positron distribution function is given by 
\begin{align}
f_{1/2} \left( p_x, p_z \right) = \frac{\mathbbm{s}^v + \mathbf{p} \cdot \boldsymbol{\mathbbm{v}}^v}{\omega} \bigg \vert_{t \to \infty} \label{equ:n}
\end{align}
and the particle number density for spinless particles is given by
\begin{align}
%f_0 \left( p_x, p_z \right) = \frac{2 \mathbbm{h}^v + \mathbf{p} \br{t}^2 \left( \mathbbm{g}^v + \mathbbm{h}^v \right) }{\omega \br{t}}. \label{equ:f}
f_0 \left( p_x, p_z \right) = \frac{2 \mathbbm{h}^v + \mathbf{p} \cdot \boldsymbol{\mathbbm{j}}^v }{\omega} \bigg \vert_{t \to \infty}. \label{equ:f}
\end{align}
%Note, that the particle spectrum at asymptotic times (vanishing vector potential) is cylindrically symmetric in $(p_x,p_y)$. Hence, it is
%perfectly fine to analyze the data for $f \left( p_x, p_z \right)$ only.
In the parameter region of interest the particle momentum spectrum at asymptotic times (vanishing vector potential) is axially symmetric in $(p_x,p_y)$. 
For the sake of simplicity, we therefore have $p_y=0$ and refer
to $p_x$ as in-plane or parallel momentum. In this regard, $p_z$ defines the perpendicular momentum.

\paragraph{Photoparticle angular distribution.--}

In order to enable multiphoton particle production the total photon energy $n \omega$ has to exceed not only the particles' rest mass but also
their oscillatory energy in the background field $2 m_\ast$. Here, $m_\ast$ describes the particle's effective mass
in a homogeneous, oscillating background field
\begin{equation}
 m_\ast = m \sqrt{1+ \xi^2 } \approx m \sqrt{1+ \frac{\varepsilon^2 m^2}{4 \omega^2} },
\end{equation}
where $\xi=\frac{e}{m} \sqrt{ -\langle A^\mu A_\mu \rangle }$.
Moreover, energy conservation laws dictate the particle's kinetic energy and as a consequence its momentum reads \cite{Kohlfurst:2013ura}
\begin{equation}
 \mathbf{p}^2_\ast = \left(\frac{n \omega}{2} \right)^2 - m_\ast^2. \label{equ:En1}
\end{equation}
From eq. \eqref{equ:En1} we can already deduce that particle distributions form shells in phase space, which can be
classified by the number of photons absorbed \cite{Otto:2014ssa}. 
The effective mass model, however, cannot explain why each shell falls off differently.

For the case under consideration it is useful to perform the partial wave analysis for the particle distribution and not the quantum amplitudes.
Within the absorption model, given a specific shell $N$ ($n$-photon absorption), the particle's angular distribution is given by \cite{Yang:1948nq}
\begin{equation}
 I \left(\vartheta, \varphi \right) \propto \sum_{L=0}^{2N} \sum_{M=-L}^L B_{LM} Y_{LM} \left(\vartheta, \varphi \right), \label{equ:I}
\end{equation}
with the coefficients $B_{LM}$, the spherical harmonics $ Y_{LM}$ and the angular momentum quantum numbers $L$ and $M$.
As our focus in this manuscript is on circularly polarized light only,
the probability distribution simplifies drastically
\begin{equation}
 I_S \left(\theta \right) = M_S \sin^{2(N-S)} \left( \theta \right), \label{I_c}
\end{equation}
where $S$ describes the total particle spin and $M_S$ states the spin-dependent creation rate. The angle
$\theta$ is defined as the angle between the field's propagation direction and the particle's ejection direction.
%and $\phi$ is the azimuthal angle.  

%$M_c$ is a function of (i) energy of incident light $\omega$ ($1/\omega / \omega^{2(N-1}$)  and (ii) beam intensity $\varepsilon^2$ ($\varepsilon^{2(N-1)}$)
%M_c check for (-1)^l dependency and absolut values



==> TeX/Introduction.tex <==
\paragraph{Introduction.--}

Photoelectron angular distributions (PAD) are well known in chemistry and atom physics, where the focus is on 
studying ionization spectra and understanding the inner structure of molecules and atoms \cite{Reid}. Viewing
multiphoton pair production as the highly relativistic analogue of the ionization of hydrogen, we
can expand the concept of angular momentum transfer via photon absorption to the strong-field QED regime.

In theory, particle production is similar to atomic ionization \cite{Brezin}, e.g., above-threshold effects in the multiphoton regime \cite{Delone:1994}.
Specifically, the particle under consideration absorbs more photons than necessary in order to transit to a continuous state, which manifests in a series of peaks in the momentum spectrum.
In both scenarios, the peak positions are determined by the number of absorbed photons and the field-dependent threshold \cite{Kohlfurst:2013ura,Lv:2018qxy,Otto:2014ssa,Akal:2014eua}.
A partial wave analysis, however, has been performed only in atomic physics, where a model for angular momentum transfer
was introduced, see Refs. \cite{Reid,IonizeH} for reviews and further information on this topic as well as Ref. \cite{PhysRevA.87.033413} for a recent experimental verification.  

% Interactions of strong laser pulses with atomic systems have much in common with theoretical studies on pair production \cite{Brezin},
% most prominently above-threshold effects in the multiphoton regime \cite{Delone:1994}. To be more specific, the particle under consideration
% absorbs more photons than necessary to transit to a continuous state leading to a series of peaks in the momentum spectrum.
% The peak positions can be quantified precisely in both scenarios accepting a field-dependent threshold (ponderomotive
% potential compared to the concept of an effective mass \cite{Kohlfurst:2013ura,Lv:2018qxy,Otto:2014ssa}), which in turn gives rise to 
% further phenomena, e.g., channel closing \cite{Kohlfurst:2013ura}.
% The interference patterns, however, have been only investigated in atomic physics, where a model for angular momentum transfer
% was introduced, see Refs. \cite{Reid,IonizeH} for reviews and further information on this topic as well as Ref. \cite{PhysRevA.87.033413} for a recent experimental verification.  

With regards to strong-field matter creation, the focus has been on understanding the different mechanism to create particles in the first
place, see Refs. \cite{Sauter:1931zz}, \cite{Breit:1934zz}, \cite{Dinu:2017uoj} and \cite{Schutzhold:2008pz}. Furthermore, in contrast to atomic ionization there has been only one successful
experiment carried out so far \cite{Burke:1997ew}. However, as laser development progresses the strong-field regime becomes more accessible, thus enabling studies on
particle creation processes on a regular basis, see Refs. \cite{Experiments, Ribeyre:2015fta} for detailed information on planned projects.

% First theoretical predictions about the possibility to convert light to matter have been published
% in the mid of the last century \cite{Sauter:1931zz}. However, due to the high field strengths needed
% progress in understanding non-linear quantum vacuum effects have been mainly of a more theoretical nature.
% Nevertheless, due to the advent of laser physics, multiphoton pair production could verified experimentally 
% \cite{Burke:1997ew}. Furthermore, nowadays various experiments are dedicated to measure particle creation through
% the Breit-Wheeler process \cite{Experiments}. In these facilities, an electron beam is used to create 
% high-energy photons ($\sim$ GeV) via bremsstrahlung, which, in turn, interact with the low-energy photons ($\sim$ eV)
% of a counter-propagating laser beam. In this article, we only consider photon interactions thus in our scenario
% we have monochromatic photon beams containing photons with energies of the order of several hundreds of kiloelectron volts.

In order to study multiphoton pair production in electric fields we compute
distribution functions using a phase-space formalism \cite{Vasak:1987umA,Heinz}. To be more specific, we work with
quantum kinetic theory (QKT) \cite{Smolyansky:1997fc}. One big advantage of QKT is, that it is easy to obtain results for
fermionic as well as bosonic pair production, since both are described by a set of time-dependent ordinary differential equations. Additionally, the
framework allows to freely choose the polarization of the laser beams \cite{Li:2015cea,Rotating,Blinne:2015zpa}. On top of that, we obtain direct access to
the particle's momentum spectrum \cite{Smolyansky:1997fc}. Such spectra are then discussed on the basis of a photon absorption model taking into account
energy and angular momentum conservation.

In this article we only consider simple, time-dependent, rotating electric fields \cite{Rotating,Blinne:2015zpa}. 
Such configurations provide the perfect setting for testing our absorption model. 
In particular, the orientation of the photon spin is fixed making selection rules much easier to apply. 

Throughout this paper we use natural units $\hbar=c=1$ and measure all dimensionful quantities in terms
of the mass of the particles $m$.








==> TeX/Results.tex <==
%\section{Results}

\paragraph{Scalar pair production.--}

      \begin{figure}[t]
      \begin{center}
	\includegraphics[width=0.45\textwidth]{Figures/fpxpz.png} 	
      \end{center}
      \caption{Scalar particle distribution function $f_0$ as a function of the in-plane momentum $p_x$ and the perpendicular momentum $p_z$ for
      a field with peak strength $\varepsilon=0.075$, frequency $\omega=0.55m$ and pulse length $\tau=250m^{-1}$.
      The shells arise due to the absorption of $4$, $4+1$ and $4+2$ photons (above-threshold pair production).}
      %Data: sQED_highres_eps75_w05
      \label{fig:fpxpz}
      \end{figure}  
      
%       \begin{figure}[t]
%       \begin{center}
% 	\includegraphics[width=0.49\textwidth]{Figures/fpx_px.png} 	
%       \end{center}
%       \caption{Log-plot of the local maxima in the spectrum $n_0 (p_{x,\ast},0)$ together with their corresponding peak location $p_{x,\ast} (\omega)$ for increasing field frequencies.
%       The above-threshold peaks seem to reach their respective maximum at a momentum of $p_x \approx 0.76$m (grey line). Due to angular momentum transfer,
%       $n$-photon pair production@ 
%       Field parameters: $\varepsilon=0.075$ and $\tau=250$m$^{-1}$.}
%       %Data: sQED_paper_eps
%       %Data2: data4(5,6,7) in sQED_paper_epsA(B,C,D)
%       \label{fig:f_px}
%       \end{figure}        

%Angular momentum effects are best discussed on the basis of particle distributions in momentum space, an example is given in Fig. \ref{fig:fpxpz} for $f_0$ with $\omega=0.55$m and $\varepsilon=0.075$. 
The shell structure as well as the lack of pronounced interference patterns can be observed in our results. In Fig. \ref{fig:fpxpz}, where we employed a background
field with peak strength $\varepsilon=0.075$, frequency $\omega=0.55m$ and pulse length $\tau=250m^{-1}$,
we recognize a perfectly regular pattern of three peaks at momenta $\mathbf{p}_4 = 0.4556m$, $\mathbf{p}_5 = 0.9419m$ and $\mathbf{p}_6 = 1.311m$. 
Here, the indices enumerate the shells with above-threshold peaks
caused by the absorption of $4$, $5$ and $6$ photons. The predictions obtained by the effective mass model yield $\mathbf{p}_{\ast,4}=0.4532m$, 
$\mathbf{p}_{\ast,5}=0.9413m$ and $\mathbf{p}_{\ast,4}=1.3107m$, which support our interpretation.

As stated above, the model for the background field \eqref{eq:A} describes photons with helicity $+1$ only. Hence, in an $n$-photon process the total angular momentum
before particle creation takes place is equal to the number of photons $n$ in the process. As angular momentum must be conserved, the total angular
momentum of the produced particle pair has to be $n$, too. Hence, every photon absorbed increases the total angular momentum of
the particles by one. As these particles do not possess an intrinsic spin the total angular momentum is equal to the pairs' orbital angular momentum $L$.
%With respect to eq. \eqref{I_c}, it is also not surprising, that the distribution function in Fig. \ref{fig:fpxpz} does not exhibit any interference pattern.

      \begin{figure}[t]
      \begin{center}
	\includegraphics[width=0.49\textwidth]{Figures/fpx_eps.png} 	
      \end{center}
      \caption{Displaying peaks in the $n$-photon production probability as a function of the background field strength $\varepsilon$ for $\omega=0.666m$ and $\tau=250m^{-1}$.
      Despite a field-dependent threshold we can monitor the local maxima in the spectrum $f_0 (p_{x,\ast},0)$ and fit a model of the form $\varepsilon^{2n}$
      to the numerical data (black lines).}
      %Data: sQED_paper_eps1
      \label{fig:f_eps}
      \end{figure}        

As we also aim to obtain a quantitative understanding of the processes, we test for non-trivial scaling of the $n$-photon peaks. 
Hence, we have solved the governing equations of scalar QKT \eqref{eq:sQED1}-\eqref{eq:sQED3} for various values of the peak field strength $\varepsilon$ 
at the effective momenta $\mathbf{p}_\ast = (p_{x,\ast},0)$ for $4$-, $5$- and $6$-photon processes, c.f. Fig. \ref{fig:f_eps}. Monitoring each peak individually
has the advantage that we can ensure we are probing a fundamental observable; in Ref. \cite{Kohlfurst:2013ura} the total yield was discussed, which suffers 
from having multiple sources of contributions. We fit a simple model of the form of $\varepsilon^{x_n}$ to the data, because
the intensity of a laser beam coincides with the number of photons in the beam $I \sim \varepsilon^{2} \propto n$.
The exponents were calculated to be $x_4=7.94$, $x_5=9.96$ and $x_6=11.96$ with confidence intervals of $(7.92, 7.95),~ (9.96, 9.97)$ and $(11.96, 11.97)$ at $95\%$ confidence.
For comparison, our model predicts an increase of $\varepsilon^{2n}$, thus de facto excluding any non-trivial effects at low field strengths. 

\paragraph{Electron-positron pair production.--}
      
      \begin{figure}[t]
      \begin{center}
	\includegraphics[width=0.49\textwidth]{Figures/ftheta.png} 	
      \end{center}
      \caption{Photoelectron angular momentum $f(\theta)$ in case of $4$-photon pair production decomposed in terms of anti-parallel ($S=0$) and parallel ($S=1$) spin contributions 
      for $\varepsilon=0.075$, $\omega=0.55m$ and $\tau=250m^{-1}$. The black lines correspond to fits of the form of $\sin^{2(4-S)} (\theta)$.
      Scalar pair production is given by the green curve (diamonds).      
      Electron-positron pair production (QED) is the sum of scalar and spin-1 contributions.}
      %Data: sQED_highres_eps75_w05
      \label{fig:ftheta}
      \end{figure}          
      
%The momentum spectra in electron-positron pair production look very similar to the spectra for scalar pair production discussed above. 
Electron-positron momentum spectra generally look similar compared to their scalar counterparts.
The differences stem from the fact that there are two options for spin alignment in a pair of spin-$1/2$ particles; parallel and anti-parallel.
In the former, both spins point in the same direction thus their total spin is given by $S=1/2+1/2=1$; while in the latter the total spin adds up to $S=0$.
Hence, in an $n$-photon absorption process there are now two options for the 
particles orbital angular momentum $L$. As a result, the model for fermionic pair production can be put in the form
% \begin{multline}
%  I \left(\theta \right) = \\
%  \varepsilon^{2n} \ \left| M_0 (\omega) \sin^{2n} \left( \theta \right) + M_1 (\omega) \sin^{2(n-1)} \left( \theta \right) \right|, \label{I_ferm}
% \end{multline}
\begin{equation}
 I \left(\theta \right) = 
 \varepsilon^{2n} \ \left| M_0 (\omega) \sin^{2n} \left( \theta \right) + M_1 (\omega) \sin^{2(n-1)} \left( \theta \right) \right|, \label{I_ferm}
\end{equation}
where $M_i$ can take on negative values. This is slightly different compared to the simpler case of scalar pair production, where no $S=1$ state exists.

One consequence of the existence of an excited spin state becomes apparent when investigating particles with vanishing momentum $\mathbf {p}$.
Every photon absorbed by the particle pair adds $+1$ to its total angular momentum. In case of scalar pair production, or if spins are aligned
anti-parallel ($S=0$), all angular momentum is carried by the quantum number $L$. As a non-zero orbital momentum requires a non-zero linear momentum,
pair production cannot happen in this case. The only option for particle creation at vanishing linear momentum $\mathbf{p}$ is a one-photon process, 
where the particle spins align parallel, thus absorbing the photon angular momentum and resulting in $L=0$.
%As in such a case the orbital angular momentum $L$ is zero, the linear momentum can be zero, too. 

Interestingly, one-photon absorption is also the only way to obtain particle ejection in the propagation direction of the laser beams. If the energy
of one and only one photon exceeds the rest energy of a fermionic particle pair, we obtain a closed shell in momentum space. This is because only 
for the one-photon process an electron-positron pair in an $S=1$ spin state can absorb all the photon angular momentum and have a 
vanishing orbital angular momentum.

%The picture we are drawing here is nicely in line with findings in Ref. \cite{Marinov:1977gq}. It was stated, that in the case of $\mathbf{p}=0$
%the particle spectrum can be understood on the basis of selection rules. Due to the fact, that CP-parity of a fermion pair with vanishing momentum is $(-1)^{S+1}$
%and due to the vacuum being CP-even, an electron-positron pair created from the vacuum has to have $S=1$.

% This observation is directly connected to particle ejection in propagation direction of the laser beams. In monochromatic, linearly polarized
% field configurations parity conservation can prevent particles with zero momentum to be formed. In a seminal article \cite{Marinov:1977gq} it was shown, that 
% fermionic pair production at $\mathbf{p}=0$ is only possible at odd photon numbers. In turn, scalar pair production at vanishing momentum requires an even number of absorbed photons.
% In following studies it was then observed, that a similar argument holds if the particle momentum is zero in polarization direction of the field.
% In circularly polarized fields, the suppression of particles production in transversal direction $p_z$ is more severe \eqref{I_c}.
% Again, the only option to create such a particle stream is given by one-photon absorption. 

% A similar observation can be made in case of particle ejection in propagation direction of the laser beams. In monochromatic, linearly polarized
% field configurations parity conservation can prevent particles with zero parallel momentum to be formed (parallel with respect to the field polarization).
% To be more specific, in such a case fermionic pair production is only possible at odd photon numbers. 
% In turn, scalar pair production at vanishing parallel momentum requires an even number of absorbed photons. 
% In circularly polarized fields, the suppression of production rates in transversal direction $p_z$ is more severe \eqref{I_c}. @
% Again, the only option to create such a particle stream is given by one-photon absorption.

Generally, there are contributions from both spin-states to the electron-positron momentum spectrum. 
%As we have already established above, for multi-cycle pulses particles form shell structures due to energy conservation. 
In this regard, it is interesting to discuss the particle spectrum as a function of the angle $\theta$, where $\theta=90^\circ$ corresponds to $(p_x,0)$, 
see Fig. \ref{fig:ftheta}.
%We have displayed the electron's angular momentum distribution function $f_{1/2} (\theta)$ in Fig. \ref{fig:ftheta}.

Solving scalar QKT for a $4$-photon event ($\varepsilon=0.075$ and $\omega=0.55m$) we obtain a particle distribution ($\mathbf{p}_\ast=0.456m$) which is
perfectly described by our model; here $\overline M_0 = 0.9987 \ (0.998, 0.999)$ with $95\%$ confidence interval and $R^2=0.999997$ using normalized quantities.
In the case of fermionic particles, we obtain a distribution function $f_{1/2} (\theta)$ with contributions from an $S=0$ as well as from an $S=1$ state.
Assuming that for a given field configuration the particle creation rates for the attainable spin states do not change (besides a trivial factor of $2$
due to combinatorics in $M_0$), we can subtract the zero-spin production probability from the total probability yielding the contribution from the $S=1$ state alone.

Applying our model to fit the data we find the numerical results being well described by a ${\rm sin}^{6}$ function, as 
we obtain $\overline M_1 = 1.01$ with confidence interval $(1.00, 1.02)$ at $95 \%$ certainty and $R^2=0.9994$.
It is remarkable to see the
contribution from the $S=1$ state being much higher than the contribution from the singlet state. In a way, this situation
resembles the status regarding orthohelium and parahelium with orthohelium ($S=1$) having a lower rest energy.



   
   
